LADIS: Language Disentanglement for 3D Shape Editing

Natural language interaction is a promising direction for democratizing 3D shape design. However, existing methods for text-driven 3D shape editing face challenges in producing decoupled, local edits to 3D shapes. We address this problem by learning disentangled latent representations that ground language in 3D geometry. To this end, we propose a complementary tool set including a novel network architecture, a disentanglement loss, and a new editing procedure. Additionally, to measure edit locality, we define a new metric that we call part-wise edit precision. We show that our method outperforms existing SOTA methods by 20% in terms of edit locality, and up to 6.6% in terms of language reference resolution accuracy. Our work suggests that by solely disentangling language representations, downstream 3D shape editing can become more local to relevant parts, even if the model was never given explicit part-based supervision.

==> sections/4_method_OLD.tex <==
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{figures/listener_architecture.png}
  \caption{Overview of the network architecture...etc. This should have both the listening and the edit-time optimization in there.}
\end{figure*}


\subsection{Problem statement}

Source,target, language triplets
Some energy function that evaluates compatibility of a shape given a source shape and language. 

\subsection{Autoencoding of 3D shapes}
This stuff background :
\begin{enumerate}
\item reconstruction-based autoencoders capture useful geometric information on a lower-dimensional space
\item interpolation within this space has shown to be meaningful (cite examples  from stuff like DSGNET) but they typically do not have controllable semantics.
\end{enumerate}

\subsection{Listening architecture}
TODO: come with a catchy name for this

This is the method by which we model this compatibility. Changes between shapes as a firt-class citizen.
 
Expert networks and techniques for getting them to specialize. 

\subsection{Language orthogonality}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/listener_architecture.png}
  \caption{Example of multiple independent utterances (within the same context)}
\end{figure}



Motivate why the geometric concept of orthogonality actually makes sense in the context of the listening architecture proposed.

This helps  editing in two different ways: semantic meaningfulness (getting the listener to perform better) and edit locality.

\subsection{Optimization-based editing}

In practice, we see two major problems: 1) generating invalid geometry, and 2) generating unnoticeable edits. For this we have two proposals.

How do we ensure that for arbitrary AE latent space, that optimization-based editing does not move off the data manifold? Answer: we use neighbors in a clever way.

How do we ensure that the "extent" of edits and directions are decoupled? Answer: we automatically calibrate the step size with regards to gradients of the decoder.


% \begin{enumerate}
% \item The listener architecture: a diagram of the architecture, with specific details on the choice of normalization, as well as the reason why the difference-space is not source-shape conditional.

% \item Implementation of the language disentanglement losses: multiutterances within Shapetalk and batchwise orthogonality.

% \item Optimization-based editing: The use of nearest neighbors for interpolation. A rough pseudocode for how the edits are done. Technique for controlling visual obviousness of change.
% \end{enumerate}

==> sections/5_experiments_OLD.tex <==



\subsection{Neural Listening}

Table 1: backbones vs. listening accuracy

\subsection{Editing}

Table 1: One number for as many backbones and datasets as possible. we're not claiming which representation is the best, the important thing is the ablations. Methods within a single backbone is directly comparable to one another.

Table 1: 3 backbones, 2 datasets, 3 or 4 methods. (b1: our method in all its glory, b2: dumb listener + sophisticated traversal, b3: dumb listener + dumb traversal , b4: sophisticated listener + dumb traversal, b5: Nearest Neighbor search) Summarizes our contributions on the listening and editing side.

Table 2: 1 backbone (IM-Net), ablate all the design decisions. 

% One-shot edits
% iterative edits

% the effect of different edit-time parameters



\subsection{Analyzing the language representation}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/listener_architecture.png}
  \caption{TSNE-plot of language embeddings in different baselines table 1.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/listener_architecture.png}
  \caption{Part segmentation as a byproduct.}
\end{figure}

\subsection{ Qualitative Editing examples}
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/listener_architecture.png}
  \caption{Qualitative results, comparing with baselines in table 1. It has to have a pair for comparison where everything else the same EXCEPT for language orthogonality.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/listener_architecture.png}
  \caption{Edit drift, language ortho helps with preserving over iterations of edits.}
\end{figure}

\begin{enumerate}

\item Listening experiments and accuracies. We will be comparing: \textbf{Ours w/ multiutterance} will be the model where we train using the orthogonality loss imposed across the multiple shapetalk utterances within the same Shapetalk context. \textbf{Ours w/ batch} will be the model where the orthogonality loss is applied across the batch instead. This shows the effectiveness of the approach in cases when you do not have information on the other utterances said about the same context. \textbf{Ours w/o orthogonality} The model without any orthogonality regularization, whether batch-wide or context-wide. \textbf{ChangeIt3D w/ IMNet} the neural listening accuracy for the ChangeIt3D listener with the IMNet backbone. \textbf{ChangeIt3D w/ ShapeGF} the accuracy of the listener that uses the diffusion-based backbone, ShapeGF. The table will show that our testing accuracy is about 3\% higher than the highest of all of these (ShapeGF), and 10\% higher than \textbf{Ours w/o orthogonality}.

\item Editing experiments -- Showing qualitative results of edits done by a selection of the above methods on Chairs and Tables. Displaying samples where our model with orthogonality loss produces more disentangled edits for fine-grained utterances, where baseline methods fail. We will also have lGD metrics using Partnet chairs, and reports of LAB scores as well. lGD scores currently show that the language orthogonality loss reduces the lGD by about 12.5\%.

\item Iterative editing -- Visualizations of the same language instruction being iteratively applied, as well as the L-GD metrics/LAB score drops/increases per step. This section seeks to show the importance of disentanglement, and the catastrophic failure that can arise from having unsolicited edits compound over iterations.

\item Visualization of language latents -- want to visualize the orthogonality of parts, and the opposites of sentences that antonymous adjectives.  Our current visualization of the language latents shows that the orthogonality loss encourages part-semantics to be developed naturally. More about this later.

\item Shape retrieval experiments.

\end{enumerate}






==> sections/5a_evalmetric_OLD.tex <==
We introduce a metric to quantify the extent to which different edits are disentangled. Designing a metric for this presents many challenges:
\begin{enumerate}
\item Since we would ideally like to measure the extent to which changes are enacted on regions of the object that are mentioned by language, we naturally have to establish some correspondence between utterances and subregions of the edited shape.
\item We want to guard against cases when the network cheats, in two ways: 1) by producing edits that produce minuscule differences \textit{everywhere}, and 2) by producing edits that fail to align better with the input utterance.
\item We additionally want to measure the extent to which "leakage" happens  to unmentioned regions of the shape throughout multiple iterative edits.
\end{enumerate}

To address both of these challenges, we propose the \textit{Edit Precision Score}, which evaluates the degree of concentration of changes to an input shape $s_0$ within a mentioned part within utterance $l$, throughout a sequence of edits defined by $s(t)$ for $t \in [0, T]$,  with $s(0) = s_0$.

We assume that for input shape $s_0$, we have a bounding-box part decomposition $R_{s_0}: \mathbb R^3 \rightarrow \mathcal P(P)$ that maps a given point in $\mathbb R^3$ to a subset of $P$, the full set of part labels.

We also construct a mapping $Q: L \rightarrow \mathcal P(P)$, which is a manually designed classifier that, based on the words within the utterance from space $L$, selects a subset of $P$ as "active" parts, where changes should be allowed.

Using $R$ and $Q$, we can define the "active" set for a given language instruction, by:
$$ \mathcal X_{(s_0, l)} = \mathcal X \cap R_{s_0}^{-1} (Q(l))$$
where $X \subset \mathbb R^3$.

Let $\mathcal D_{\mathcal X} (s, s')$ and $\mathcal D_{\mathcal X_{(s_0, l)}} (s, s')$ denote some geometric distance $\mathcal D$ restricted on certain subsets $\mathcal X_{(s_0, l)}$ and $\mathcal X$ of $\mathbb R^3$. For different geometric representations, the choice for $\mathcal X$ and $\mathcal D$ may vary. For implicit representations, for instance, we will be using $\mathcal X = \mathbb R^3$ and
$$ \mathcal D_A(s, s')  = \int_{x \in A}|d(s, x) - d(s', x)| d x $$ where $d$ is the pretrained implicit decoder for query point $s$.

As such, we can define the \textbf{precision} of a single edit $s'$, $P(s_0, s', l)$, by:

$$ P(s_0, s', l) = \frac{\mathcal D_{\mathcal X_{(s_0, l)}} (s_0, s')}{\mathcal D_{\mathcal X}(s_0, s')}$$

Then we let the measurement of edit precision $CEP(s(t), l)$ be defined as:
$$ \int_{0}^{T} P(s_0, s(t), l) \max(\phi(s_0, s(t), l), 0) dt$$

where $\phi : S \times S \times L \rightarrow [-1, 1]$  is the listener, and $T$ is the length of the edit sequence.

To evaluate this metric, we manually design a mapping from a subset of words used within the utterances of the dataset and part classes of chairs within the PartNet dataset.

